TempoFormer: A Transformer for Temporally-aware Representations in Change Detection

Dynamic representation learning plays a pivotal role in understanding the evolution of linguistic content over time. On this front both context and time dynamics as well as their interplay are of prime importance. Current approaches model context via pre-trained representations, which are typically temporally agnostic. Previous work on modelling context and temporal dynamics has used recurrent methods, which are slow and prone to overfitting. Here we introduce TempoFormer, the first task-agnostic transformer-based and temporally-aware model for dynamic representation learning. Our approach is jointly trained on inter and intra context dynamics and introduces a novel temporal variation of rotary positional embeddings. The architecture is flexible and can be used as the temporal representation foundation of other models or applied to different transformer-based architectures. We show new SOTA performance on three different real-time change detection tasks.

==> extras.tex <==
\begin{table*}[t]
\begin{adjustbox}{max width=\textwidth,center}
\begin{tabular}{{|c|cccc|ccc|cccc|ccc|}}
\hline
 & \multicolumn{4}{|c|}{\textbf{AnnoMI}} & \multicolumn{3}{|c|}{\textbf{LRS}}
 & \multicolumn{4}{|c|}{\textbf{TalkLife}} & \multicolumn{3}{|c|}{\textbf{Topic Shift}} \\
 
\textbf{window} &N & C & S & avg      & N-Sw & Sw & avg     & IE & IS & O&avg      & M & R & avg \\\cline{1-15}

\parbox[t]{2mm}{\multirow{1}{*}{5}}&74.1 &48.8&35.0&  52.6 & 70.5&54.7& 62.6& 50.1& 28.3 &88.8 & 55.7 &38.5& 69.7 &54.1\\

\midrule
\bottomrule

\parbox[t]{2mm}{\multirow{1}{*}{10}}&75.4 &48.0&35.5& 53.0 & 73.2&56.2& 64.7& 50.2& 32.6 &88.5 & 57.1 &40.0& 70.8 &55.4 \\
\midrule
\bottomrule

\parbox[t]{2mm}{\multirow{1}{*}{20}}&75.4 &48.8&35.9& 53.4 &75.4& 60.2& 67.8& 50.1 &31.9 &88.5 & 56.8 &40.4& 70.1 &55.3 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Macro-average scores on all datasets for different window sizes. \textbf{Best} window scores are marked. All based on a single seed as of now. 4-seeds for AnnoMI(w-5),5-seeds for AnnomI(w-10), 5-seeds for AnnomI(w-20), 5-seeds for LRS(w-5),5-seeds for LRS(w-10),5-seeds for LRS(w-20),5-seeds for TLife(w-5)}
\label{extras}
\end{table*}



\begin{table*}[t]
\begin{adjustbox}{max width=\textwidth,center}
\begin{tabular}{{|c|ccc|cccc|ccc|}}
\hline
& \multicolumn{3}{|c|}{\textbf{LRS}}
 & \multicolumn{4}{|c|}{\textbf{TalkLife}} & \multicolumn{3}{|c|}{\textbf{Topic Shift}} \\
 
\textbf{window} & N-Sw & Sw & avg     & IE & IS & O&avg      & M & R & avg \\\cline{1-11}

\parbox[t]{2mm}{\multirow{1}{*}{5}}& 70.5&54.7& 62.6& 50.1& 28.3 &88.8 & 55.7 &39.4& 69.6 &54.5\\

\midrule
\bottomrule

\parbox[t]{2mm}{\multirow{1}{*}{10}}& 73.2&56.2& 64.7& \textbf{50.2}& \textbf{32.6} &\textbf{88.5} & \textbf{57.1} &40.0& \textbf{70.8} &\textbf{55.4} \\
\midrule
\bottomrule

\parbox[t]{2mm}{\multirow{1}{*}{20}} &\textbf{75.4}& \textbf{60.2}& \textbf{67.8}& 50.1 &31.9 &\textbf{88.5} & 56.8 &\textbf{40.4}& 70.1 & 55.3 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Macro-average scores on all datasets for different window sizes. \textbf{Best} window scores are marked. All based on a single seed as of now. 5-seeds for LRS(w-5),5-seeds for LRS(w-10),5-seeds for LRS(w-20),5-seeds for TLife(w-5), 5-seeds for TS(w-5), 5-seeds for TS(w-10). All on lichfield.}
\label{extras2}
\end{table*}

